Rule-based Graph Repair

Model repair is an essential topic in model-driven engineering. Since models are suitably formalized as graph-like structures, we consider the problem of rule-based graph repair: Given a rule set and a graph constraint, try to construct a graph program based on the given set of rules, such that the application to any graph yields a graph satisfying the graph constraint. We show the existence of repair programs for specific constraints, and show the existence of rule-based repair programs for specific constraints compatible with the rule set.

==> eptcsdata.tex <==
\providecommand{\firstpage}{87}
\providecommand{\publicationstatus}{Rachid Echahed and Detlef Plump (Eds.): Tenth International\\ Workshop on Graph Computation Models (GCM 2019)\\
EPTCS 309, 2019, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.309.5}{10.4204/EPTCS.309.5}}

